Transfer Learning of an Ensemble of DNNs for SSVEP BCI Spellers without User-Specific Training

Objective: Steady-state visually evoked potentials (SSVEPs), measured with EEG (electroencephalogram), yield decent information transfer rates (ITR) in brain-computer interface (BCI) spellers. However, the current high performing SSVEP BCI spellers in the literature require an initial lengthy and tiring user-specific training for each new user for system adaptation, including data collection with EEG experiments, algorithm training and calibration (all are before the actual use of the system). This impedes the widespread use of BCIs. To ensure practicality, we propose a highly novel target identification method based on an ensemble of deep neural networks (DNNs), which does not require any sort of user-specific training. Method: We exploit already-existing literature datasets from participants of previously conducted EEG experiments to train a global target identifier DNN first, which is then fine-tuned to each participant. We transfer this ensemble of fine-tuned DNNs to the new user instance, determine the k most representative DNNs according to the participants' statistical similarities to the new user, and predict the target character through a weighted combination of the ensemble predictions. Results: On two large-scale benchmark and BETA datasets, our method achieves impressive 155.51 bits/min and 114.64 bits/min ITRs. Code is available for reproducibility: https://github.com/osmanberke/Ensemble-of-DNNs Conclusion: The proposed method significantly outperforms all the state-of-the-art alternatives for all stimulation durations in [0.2-1.0] seconds on both datasets. Significance: Our Ensemble-DNN method has the potential to promote the practical widespread deployment of BCI spellers in daily lives as we provide the highest performance while enabling the immediate system use without any user-specific training.

==> ref <==
\begin{thebibliography}{10}

\bibitem{Sellers257re7}
E.~W. Sellers, D.~B. Ryan, and C.~K. Hauser, ``Noninvasive brain-computer
  interface enables communication after brainstem stroke,'' {\em Science
  Translational Medicine}, vol.~6, no.~257, pp.~257re7--257re7, 2014.

\bibitem{BCI-base}
S.~Dutta, T.~Banerjee, N.~Dutta~Roy, B.~Chowdhury, and A.~Biswas, ``Development
  of a bci-based gaming application to enhance cognitive control in psychiatric
  disorders,'' {\em Innovations in Systems and Software Engineering}, 08 2020.

\bibitem{10.3389/fnins.2010.00198}
B.~Blankertz, M.~Tangermann, C.~Vidaurre, S.~Fazli, C.~Sannelli, S.~Haufe,
  C.~Maeder, L.~Ramsey, I.~Sturm, G.~Curio, and K.~Mueller, ``The berlin
  brain–computer interface: Non-medical uses of bci technology,'' {\em
  Frontiers in Neuroscience}, vol.~4, p.~198, 2010.

\bibitem{kerous}
B.~Kerous, F.~Skola, and F.~Liarokapis, ``Eeg-based bci and video games: a
  progress report,'' {\em Virtual Reality}, vol.~22, no.~2, p.~119–135, 2017.

\bibitem{6807693}
E.~{Yin}, Z.~{Zhou}, J.~{Jiang}, Y.~{Yu}, and D.~{Hu}, ``A dynamically
  optimized ssvep brain–computer interface (bci) speller,'' {\em IEEE
  Transactions on Biomedical Engineering}, vol.~62, no.~6, pp.~1447--1456,
  2015.

\bibitem{Chen_2015}
X.~Chen, Y.~Wang, S.~Gao, T.-P. Jung, and X.~Gao, ``Filter bank canonical
  correlation analysis for implementing a high-speed {SSVEP}-based
  brain{\textendash}computer interface,'' {\em Journal of Neural Engineering},
  vol.~12, p.~046008, jun 2015.

\bibitem{4203016}
Z.~{Lin}, C.~{Zhang}, W.~{Wu}, and X.~{Gao}, ``Frequency recognition based on
  canonical correlation analysis for ssvep-based bcis,'' {\em IEEE Transactions
  on Biomedical Engineering}, vol.~54, no.~6, pp.~1172--1176, 2007.

\bibitem{arxivpaper}
O.~B. Guney, M.~Oblokulov, and H.~Ozkan, ``A deep neural network for
  ssvep-based brain-computer interfaces,'' {\em IEEE Transactions on Biomedical
  Engineering}, early access. 2021. doi: 10.1109/TBME.2021.3110440

\bibitem{benchmark_Dataset}
Y.~{Wang}, X.~{Chen}, X.~{Gao}, and S.~{Gao}, ``A benchmark dataset for
  ssvep-based brain–computer interfaces,'' {\em IEEE Transactions on Neural
  Systems and Rehabilitation Engineering}, vol.~25, no.~10, pp.~1746--1752,
  2017.

\bibitem{beta}
B.~Liu, X.~Huang, Y.~Wang, X.~Chen, and X.~Gao, ``Beta: A large benchmark
  database toward ssvep-bci application,'' {\em Frontiers in Neuroscience},
  vol.~14, p.~627, 2020.

\bibitem{trca}
M.~{Nakanishi}, Y.~{Wang}, X.~{Chen}, Y.~{Wang}, X.~{Gao}, and T.~{Jung},
  ``Enhancing detection of ssveps for a high-speed brain speller using
  task-related component analysis,'' {\em IEEE Transactions on Biomedical
  Engineering}, vol.~65, no.~1, pp.~104--112, 2018.

\bibitem{1499837}
{Wang Yijun}, {Wang Ruiping}, {Gao Xiaorong}, and {Gao Shangkai},
  ``Brain-computer interface based on the high-frequency steady-state visual
  evoked potential,'' in {\em International Conference on Neural Interface and
  Control}, pp.~37--39, 2005.

\bibitem{MEC}
O.~{Friman}, I.~{Volosyak}, and A.~{Graser}, ``Multiple channel detection of
  steady-state visual evoked potentials for brain-computer interfaces,'' {\em
  IEEE Transactions on Biomedical Engineering}, vol.~54, no.~4, pp.~742--750,
  2007.

\bibitem{CCA_method}
Z.~Lin, C.~Zhang, W.~Wu, and X.~Gao, ``Frequency recognition based on canonical
  correlation analysis for ssvep-based bcis,'' {\em IEEE Transactions on
  Biomedical Engineering}, vol.~53, no.~12, pp.~2610--2614, 2006.

\bibitem{mec-cca-comp}
W.~Nan, C.~M. Wong, B.~Wang, F.~Wan, P.~U. Mak, P.~I. Mak, and M.~I. Vai, ``A
  comparison of minimum energy combination and canonical correlation analysis
  for ssvep detection,'' {\em IEEE/EMBS International Conference on Neural
  Engineering}, pp.~469--472, 2011.

\bibitem{to_train}
R.~Zerafa, T.~Camilleri, O.~Falzon, and K.~Camilleri, ``To train or not to
  train? a survey on training of feature extraction methods for ssvep-based
  bcis,'' {\em Journal of Neural Engineering}, vol.~15, 06 2018.

\bibitem{itr_cite}
J.~R. Wolpaw, N.~Birbaumer, D.~J. McFarland, G.~Pfurtscheller, and T.~M.
  Vaughan, ``Brain–computer interfaces for communication and control,'' {\em
  Clinical Neurophysiology}, vol.~113, no.~6, pp.~767--791, 2002.

\bibitem{fatigue}
X.~Zheng, G.~Xu, Y.~Zhang, R.~Liang, K.~Zhang, Y.~Du, J.~Xie, and S.~Zhang,
  ``Anti-fatigue performance in ssvep-based visual acuity assessment: A
  comparison of six stimulus paradigms,'' {\em Frontiers in Human
  Neuroscience}, vol.~14, 2020.

\end{thebibliography}
